Two-loop master integrals for a planar and a non-planar topology relevant for single top production

We provide analytic results for two-loop four-point master integrals with one massive propagator and one massive leg relevant to single top production. Canonical bases of master integrals are constructed and the Simplified Differential Equations approach is employed for their analytic solution. The necessary boundary terms are computed in closed form in the dimensional regulator, allowing us to obtain analytic results in terms of multiple polylogarithms of arbitrary transcendental weight. We provide explicit solutions of all two-loop master integrals up to transcendental weight six and discuss their numerical evaluation for Euclidean and physical phase-space points.

==> ApB.tex <==
\section{Numerical results up to $\mathcal{O}(\epsilon^4$}
We show numerical results up to $\mathcal{O}(\epsilon^4)$ for all top-sector canonical master integrals for the first Euclidean as well the first physical point, as defined in Table \ref{tab:points}.

\paragraph{Family $\textbf{PL1}$}

\begin{table}[h!]
    \centering
    \begin{tabular}{c||c|c|c|c|c}
                 & $\epsilon^0$ & $\epsilon^1$ & $\epsilon^2$ & $\epsilon^3$ & $\epsilon^4$ \\
                 \hline
                 \hline
       $g_{29}$   &  0 &  0 &  -0.1916387559 &  1.857186048 & -10.01082925\\
       \hline
       $g_{30}$  & $1/4$ & -2.817487622 & 15.95471394 & -57.46901214 & 143.3537514 \\
       \hline
       $g_{31}$  & $-1/4$  & 2.817487622 & -17.48654563 & 73.01716166 &  -223.0371366
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}
